Blind-date Conversation Joining

We focus on a form of joining conversations among multiple parties in service-oriented applications where a client may asynchronously join an existing conversation without need to know in advance any information about it. More specifically, we show how the correlation mechanism provided by orchestration languages enables a form of conversation joining that is completely transparent to clients and that we call 'blind-date joining'. We provide an implementation of this strategy by using the standard orchestration language WS-BPEL. We then present its formal semantics by resorting to COWS, a process calculus specifically designed for modelling service-oriented applications. We illustrate our approach by means of a simple, but realistic, case study from the online games domain.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{A. Ravara and J. Silva (Eds.): 9th Workshop on\\
Automated Specification and Verification of Web Systems (WWV'13)\\
EPTCS 123, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.123.3}{10.4204/EPTCS.123.3}}
\pdfoutput=1

